Detection of Technical Debt in Java Source Code

Technical debt (TD) describes the additional costs that emerge when developers have opted for a quick and easy solution to a problem, rather than a more effective and well-designed, but time-consuming approach. Self-Admitted Technical Debts (SATDs) are a specific type of technical debts that developers intentionally document and acknowledge, typically via textual comments. While these comments are a useful tool for identifying TD, most of the existing approaches focus on capturing tokens associated with various categories of TD, neglecting the rich information embedded within the source code. Recent research has focused on detecting SATDs by analyzing comments, and there has been little work dealing with TD contained in the source code. In this study, through the analysis of comments and their source code from 974 Java projects, we curated the first ever dataset of TD identified by code comments, coupled with its code. We found that including the classified code significantly improves the accuracy in predicting various types of technical debt. We believe that our dataset will catalyze future work in the domain, inspiring various research related to the recognition of technical debt; The proposed classifiers may serve as baselines for studies on the detection of TD.

==> src/Experiment-backup.tex <==
% \section{Experiment and Evaluation}
% \label{sec:exp_and_eval}


%\subsection{Data Pipeline Effectiveness}

%\begin{mytcbox}{\textbf{RQ1}}
%Does our pipeline extract informative examples capable of enriching the existing dataset for TD detection using code comments?
%\end{mytcbox}

We present and discuss the experimental results by addressing the research questions outlined in Section~\ref{sec:introduction}. Our study aims to develop an automated method for detecting technical debts in source code. To achieve this, we introduce a data pipeline process designed to enhance existing datasets with self-admitted technical debt comments. Our goal is to improve both the quality and variety of different types of technical debts found in comments. We then demonstrate that the enhanced dataset improves the performance of existing SATD classification models (RQ1). The augmented SATD comments are subsequently used to extract code fragments, based on the assumption that blocks of code following SATD comments will contain technical debts. The second research question (RQ2) seeks to assess the significance of source code in detecting SATD comments. We will use the source code following the comments as supplementary features to aid in identifying SATD comments.
Lastly, we assess the effectiveness of various models in identifying technical debts from source code without relying on SATD comments. Our goal is to utilize the curated dataset to detect the presence of different types of technical debts within the source code (RQ3).
In the remainder of this section, we detail the motivation, approach, and results for each of our research questions.



\subsection{\rqone}
\label{sec:RQ1}

\noindent \textbf{Motivation:} 
Existing data collection efforts for TD detections have been limited to a single phase, resulting in a relatively small corpus. This limitation has hindered the depth and diversity of the dataset, constraining the efficacy of subsequent analyses and models.  Furthermore, there is an essential need to strategically select high-value data samples for labeling to mitigate the significant human costs associated with manual annotation. We introduce a pipeline designed to gather high-value data with source code context, which we elaborate on in Section \ref{sec:Approach}. In this RQ, we focus on evaluating the effectiveness of our proposed data pipeline. 

\noindent \textbf{Approach:} We identify that the efficacy of the proposed pipeline is attributed to three fundamental modules: the \textit{SATD detection tool}, \textit{Sampling strategy}, and \textit{Annotation}. Specifically, we utilize the TD labels assigned to the comments as the standard for assessment. The detection tool is instrumental in ensuring the collection of data that contains technical debt (TD), thereby mitigating the predominance of Non-SATD data. The Sampling module is meticulously designed to identify and select high-value data, while the Annotation module is imperative for the precise and accurate labeling assignment. Therefore, our approach is to assess these modules. In particular, we leverage the final labeled data as the ground truth for evaluation.


$\sbullet[.75]$ \textbf{\textit{SATD detection tool:}} We evaluate its performance by measuring the number of comments accurately identified as containing TD. Specifically, within the \TS, the tool detected 1550 potential comments indicating TD, of which 1451 samples ($93.61\%$) are aligned with annotators. As a result, the proportion of comments containing TD in \TS increases to over $29\%$, in contrast to $6.5\%$ in \Maldonado, which lacked prior selection. These findings underscore the SATD detection tool's efficacy in identifying comments that contain TD as required.

$\sbullet[.75]$ \textbf{\textit{Annotation process:}} As detailed in Section \ref{sec:data_annotation}, we provide several steps to ensure process quality, including annotator training, a cross-check review process, and refinement through label auditing. To guarantee the reliability of the labeling process, we assess it using two consensus metrics: Raw Agreement and Inter-Annotator Agreement.

\begin{enumerate}
\item Raw Agreement: refers to the count of items for which both annotators assign identical labels, expressed as a percentage of the total items to be annotated \cite{artstein2017inter}.
\item Inter-Annotator Agreement (IAA): We employ Cohen's Kappa coefficient \citep{landis1977measurement, emam1999benchmarking}, a metric that can quantify the agreement or consistency between annotations made by different annotators.
\end{enumerate}






\begin{table}[h]
%\small
\centering
\caption{Annotation Assessment.}
\begin{adjustbox}{width=0.48\textwidth}
\begin{tabular}{l|c|c|c}
\hline
Phase & Number of comments & Raw Agreement & Inter-Annotator Agreement \\
\hline
1 & 1,400 & 56.18 & 37.00 \\
2 & 3,680 & 92.77 & 45.29 \\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:annotation_scores}
\end{table}






\begin{table*}[t]
\centering
\caption{Performance of various models on \Maldonado in three SATD related tasks (F1-score).}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{l|c|c|c|c|c|c}
\hline
& \multicolumn{2}{c|}{Identification} &  \multicolumn{2}{c|}{Classification} &  \multicolumn{2}{c}{Detection}\\
\cline{2-7}
Model & \Maldonado & +\TS ($\Delta$) & \Maldonado & +\TS ($\Delta$) & \Maldonado & +\TS ($\Delta$) \\
\hline %\hline
% DebtHunter & & & & & \\
BERT & 87.96 & 88.99 ({\color{darkgreen} +1.03}) & 51.42 & 55.10 ({\color{darkgreen} +3.68}) & 45.99 & 49.64  ({\color{darkgreen} +3.65}) \\
RoBERTa & \textbf{89.06} & 89.96 ({\color{darkgreen} +0.90}) & 53.91 & 55.32 ({\color{darkgreen} +1.41}) & 46.13 & 52.86 ({\color{darkgreen} \textbf{+6.73}}) \\
UniXCoder & 88.38 & 88.42 ({\color{darkgreen} +0.04}) & 54.82 & 54.99  ({\color{darkgreen} +0.17}) & 50.94 & 52.11 ({\color{darkgreen} +1.17}) \\
CodeBERT & 88.74 & \textbf{90.06} ({\color{darkgreen} \textbf{+1.32}}) & \textbf{57.50} & \textbf{63.70} ({\color{darkgreen} \textbf{+6.20}}) & \textbf{53.79} & \textbf{55.60} ({\color{darkgreen} +1.81})\\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:rq1}
\end{table*}

Table \ref{tab:annotation_scores} presents the annotation scores across two phases. In the initial phase, as annotators are first acquainted with the data domain, it witnesses a relatively low agreement strength of 37\%, referring to a \textit{Fair} agreement. However, following review and discussion, the agreement strength improved significantly. In the second phase, the Raw Agreement increased by over 35\%, and the IAA improved by 8\%, resulting in a \textit{Moderate} agreement strength.



$\sbullet[.75]$ \textbf{\textit{Sampling strategy:}} The sampling strategy plays a crucial role in selecting informative data samples for annotation. To measure its effectiveness, we conduct experiments on TD detection to observe the improvement achieved by incorporating \TS into the initial data source (\Maldonado) for model training. This experiment not only evaluates the Sampling strategy but also assesses the effectiveness of the general pipeline including the detection tool and annotation process.  

Experiment setup: We employ a cross-project approach following previous works \citep{da2017using, ren2019neural, sala2021debthunter, sheikhaei2024empirical}. Since \Maldonado contains 10 projects corresponding to 10-fold validation, each fold involves designating one project for testing while utilizing the other nine for model training. To prevent data leakage, we perform deduplication across the entire dataset before splitting it into 10 folds, resulting in the remaining 38,269 samples. We analyze the differences that arise when incorporating \TS during training compared to using only the base dataset - \Maldonado. We experiment with various architectures, such as BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, CodeBERT \cite{DBLP:conf/emnlp/FengGTDFGS0LJZ20} and UniXCoder \cite{DBLP:conf/acl/GuoLDW0022}, across three scenarios: SATD identification, SATD classification and SATD detection.
\begin{enumerate}
    \item SATD identification: the task involves determining whether a comment contains technical debt or not.
    \item SATD classification: requires categorizing comments containing SATD into one of five TD categories. 
    \item SATD detection: integrates both identification and classification, assigning each comment to one of six categories: five corresponding to different types of TD and one representing NonSATD.
\end{enumerate}

Due to the significant imbalance of the dataset among classes, we leverage the F1 score for performance evaluation. Table \ref{tab:rq1} presents the performance of multiple models across the three SATD tasks. By exploring a diverse array of models, we offer a holistic assessment of our pipeline's adaptability across various architectures, thereby showcasing its robustness in acquiring informative data. Overall, in all scenarios, the incorporation of \TS substantially enhances the performance across all models. In the identification and detection scenarios, the addition of new data (\TS) constituted merely 11\% of the original dataset. Nevertheless, this resulted in an enhancement of the F1 score by up to 1.32\% and 6.73\%, respectively. In general, \TS enhances the robustness of the training dataset across various models. In these two scenarios, the dataset exhibits significant imbalance, with NonSATD data comprising over 90\% of the total. The improvement underscores the effectiveness of the selected samples in addressing the issue of data imbalance. Moreover, in the SATD detection, BERT and RoBERTa exhibit inferior performance relative to the other two CodeLMs. 
However, incorporating \TS during the training phase significantly enhances the performance of these two models, resulting in comparable outcomes among all the models tested. A similar observation is presented in the classification task, where all models demonstrate improved performance when utilizing \TS. Especially, CodeBERT exhibits the highest performance across all scenarios, suggesting the advantage of using a CodeLM for comment classification tasks.

\begin{tcolorbox}[colback=gray!5!white,colframe=darkgray,title=Answer to RQ1: Data Pipeline Effectiveness]
\begin{itemize}[leftmargin=*]
    \item The SATD detection tool effectively identifies comments containing TD types, achieving an accuracy of 93.61\%. 
    \item A well-designed annotation process, including a thorough review phase, substantially enhances the labeling quality of annotators across phases. As a result, the Raw Agreement reached nearly 93\%, and the Inter-Annotator Agreement exceeded 45\%, indicating a Moderate level of agreement.
    \item Experimental results across multiple scenarios and models indicate a significant improvement when \TS is incorporated into the training process. This confirms the effectiveness of our data pipeline in selecting informative samples and annotation process.
\end{itemize}
\end{tcolorbox}

% \begin{table*}[t]
% \scriptsize
% \centering
% \caption{Performance of RoBERTa on Maldonado dataset \cite{maldonado2015detecting}.}
% \begin{adjustbox}{width=0.7\textwidth}
% \begin{tabular}{l|c|c|c|c}
% \hline
% & \multicolumn{2}{c|}{Maldonado dataset} &  \multicolumn{2}{c}{+ Tesoro} \\
% \cline{2-5}
% Project & Accuracy & F1 & Accuracy & F1\\
% \hline
% jruby-1 & 75.60	& 47.56 & 74.93 & 50.57\\
% sql12 & 80.90 & 54.56 &	82.49 & 67.41 \\
% jfreechart-11 & 73.47 & 46.46 & 73.98 & 46.81 \\
% emf-2 & 80.71 &	63.15 & 80.00 & 65.06 \\
% jEdit-4 & 85.13	& 73.10	& 85.37	& 67.51 \\
% apache-jmeter-2 & 79.45	& 50.69 & 83.94 & 69.52 \\
% columnba-1 & 71.92	& 55.93	& 78.85	& 76.11 \\
% apache-ant-1 & 80.47 & 67.94 & 80.00 &	60.40 \\
% hibernate-distribution-3 & 79.19	& 41.77	& 82.70 & 54.30 \\
% argouml & 75.46 & 51.91	& 77.31 & 55.28 \\
% \hline
% Average & 78.23 & 55.31	&\textbf{80.20}	&\textbf{60.48} \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:rq1_roberta}
% \end{table*}


% \begin{table*}[t]
% \scriptsize
% \centering
% \caption{Performance of CodeBERT on Maldonado dataset \cite{maldonado2015detecting}.}
% \begin{adjustbox}{width=0.7\textwidth}
% \begin{tabular}{l|c|c|c|c}
% \hline
% & \multicolumn{2}{c|}{Maldonado dataset} &  \multicolumn{2}{c}{+ Tesoro} \\
% \cline{2-5}
% Project & Accuracy & F1 & Accuracy & F1\\
% \hline
% jruby-1 & 78.27	& 68.70 & 77.47 & 55.58 \\
% sql12 & 81.70 & 70.44 &	83.55 & 73.16 \\
% jfreechart-11 & 77.04 & 51.13 & 76.53 & 48.78 \\
% emf-2 & 78.57 &	63.33 & 79.29 & 67.61 \\
% jEdit-4 & 85.37	& 70.37	& 84.65	& 68.47 \\
% apache-jmeter-2 & 81.35	& 59.44 & 82.56 & 63.41 \\
% columnba-1 & 77.69	& 73.51	& 79.62	& 78.10 \\
% apache-ant-1 & 79.07 & 54.66 & 79.53 &	58.69 \\
% hibernate-distribution-3 & 80.14	& 52.16	& 81.22 & 74.63 \\
% argouml & 74.27 & 53.89	& 76.55 & 60.23 \\
% \hline
% Average & 79.35 & 61.76	&\textbf{80.26}	&\textbf{64.31} \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:rq1_codebert}
% \end{table*}




\subsection{\rqtwo}
\label{sec:RQ2}

\textbf{Motivation:} Previous work on TD detection has often overlooked the inclusion of source code information, focusing primarily on comments and other textual data \citep{maldonado2015detecting,da2017using, li2023automatic, 9226330, sala2021debthunter}. However, various types of TD, such as DESIGN, IMPLEMENTATION, DEFECT, and TEST, signify intrinsic problems embedded in the source code. For example, DESIGN and IMPLEMENTATION imply poor or missing implementation within the source code. Therefore, the source code can serve as crucial information for detecting technical debt. Furthermore, from a human perspective, the annotation process (Section \ref{sec:RQ1}) demonstrates that annotators can more accurately assign TD types while incorporating the source code information. Hence, we investigate the inclusion of source code in the TD detection in this RQ.

\noindent \textbf{Approach:} We evaluate the effectiveness of various models in detecting TD by comparing their performance when utilizing only comments against when incorporating both comments and source code. To ensure a comprehensive evaluation, we designed the experiment based on the following criteria.
\begin{itemize}
    \item \textit{Model versatility:} This investigates the impact of incorporating additional source code information on different models to illustrate the broad ability of this approach. Specifically, we apply four language models.
    \item \textit{Scope of code context:} From our observations during the labeling process, annotators do not require reading the entire source code to annotate the type of TD for a comment; instead, they only need to scan the surrounding code. Based on this perspective, we explore the impact of the scope of the code context used. Specifically, we examine the effect of using the code surrounding a comment by including 2, 10, and 20 lines, as well as the entire code. Figure \ref{fig:code_context} illustrates the code context used.
    \item \textit{Integration techniques:} This setting explores several approaches for incorporating source code in detecting TD within comments. In particular, we propose two methods for investigation.
    \begin{enumerate}
        \item String Concatenation (StrConcat): Concatenate the comment with the code context to form the input string for the models.
        \item Code Attention (CodeAtt):
    \end{enumerate}
\end{itemize}




%\subsection{Source Code Effectiveness}


%\begin{mytcbox}{\textbf{RQ2}}
%Is the inclusion of source code information important in enhancing SATD detection capability?
%\end{mytcbox}




\begin{table}[h]
\scriptsize
\centering
\caption{Performance of CodeBERT on SATD detection using source code information.}
\begin{adjustbox}{width=0.4\textwidth}
\begin{tabular}{l|c|c}
\hline
Model & Accuracy & F1 \\
\hline
CodeBERT & 88.18 & 72.75 \\
\hline
CodeBERT & & \\
$\quad_{+ \text{2 code lines}}$ & 88.39 & 74.47 \\
$\quad_{+ \text{10 code lines}}$ & 88.14 & 72.08 \\
$\quad_{+ \text{20 code lines}}$ & 88.15 & 72.13 \\
$\quad_{+ \text{full code function}}$ & \textbf{88.51} & \textbf{74.80} \\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:PredictionCodeBERT}
\end{table}






\begin{table}[h!]
\centering
%\scriptsize
\caption{Performance comparison of different models on SATD detection using only comments versus additional source code information (F1-score) on \TS. The foot numbers indicate the number of context lines that achieved the best results, where $X$ represents the use of the entire code.}
\begin{adjustbox}{width=0.48\textwidth}
\begin{tabular}{l|ccc}
\hline
%\toprule
\multirow{2}{*}{Model} & Comment & \multicolumn{2}{c}{Comment + Code} \\ 
\cline{3-4}
& only & StrConcat & CodeAtt \\
\hline
RoBERTa & 68.28	& & $69.45_2$ ({\color{darkgreen} +1.17}) \\
CodeBERT & 72.75 & $76.30_X$ ({\color{darkgreen} +3.55}) & $74.80_X$ ({\color{darkgreen} +2.05})\\
UniXCoder & 70.62 & $71.54_{20}$ ({\color{darkgreen} +0.92}) & $71.46_X$ ({\color{darkgreen} +0.84}) \\ 
GraphCodeBERT & 71.39 & $74.86_2$ ({\color{darkgreen} +3.47}) & $72.75_X$ ({\color{darkgreen} +1.36}) \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:rq2}
\end{table}







\begin{tcolorbox}[colback=gray!5!white,colframe=darkgray,title=Answer to RQ2]
\begin{itemize}[leftmargin=*]
    \item Conclusions go here. 
\end{itemize}
\end{tcolorbox}


\subsection{\rqthree}


\begin{tcolorbox}[colback=gray!5!white,colframe=darkgray,title=Answer to RQ3]
\begin{itemize}[leftmargin=*]
    \item Conclusions go here. 
\end{itemize}
\end{tcolorbox}



%\subsection{TD detection in Source Code}



%\begin{mytcbox}{\textbf{RQ3}}
%How do different models perform in detecting TD types in source code when self-admitted information (comments) is absent?
%\end{mytcbox}





%\begin{table}[h]
%\scriptsize
%\centering
%\caption{Performance of various models on TD detection in source code.}
%\begin{adjustbox}{width=0.46\textwidth}
%\begin{tabular}{l|c|c}
%\hline
%Model & EM & F1 \\
%\hline
%CodeBERT & 38.28 & \textbf{43.37} \\
%UniXCoder & 38.12 & 42.58 \\
%Roberta & 35.37	& 38.22 \\
%ALBERT & \textbf{39.32} & 41.99 \\
%CodeT5+ & 37.91	& 41.96 \\
%Codellama-7b & 34.57	& 36.98 \\
%\hline
%\end{tabular}
%\end{adjustbox}
%\label{tab:rq3}
%\end{table}





\begin{table}[h!]
\centering
%\small
%	\footnotesize
\caption{Performance of various models on TD detection in source code.}
\begin{tabular}{l|cc}%|ccc|ccc|ccc|ccc}
\hline
%\toprule
Model & EM & F1 \\ \hline
%\multicolumn{3}{c}{\textbf{Average}} \\ \hline
%\cline{2-4} & 
%R--1 & R--2 & R--L\\ \hline
CodeBERT \cite{DBLP:conf/emnlp/FengGTDFGS0LJZ20} &38.28	& \textbf{43.37}  \\
UniXCoder \cite{DBLP:conf/acl/GuoLDW0022} & 38.12	& 42.58	 \\
GraphCodeBERT \cite{guo2020graphcodebert} & 39.38 & 44.21 \\
RoBERTa \cite{liu2019roberta}  & 35.37	& 38.22	 \\
ALBERT \cite{lan2019albert} & \textbf{39.32} & 41.99 \\
CodeT5+ \cite{wang2023codet5+} & 37.91	& 41.96	 \\ %\hline
CodeLlama-7b \cite{roziere2023code} & 34.57 & 36.98	 \\
\hline
\end{tabular}      
\label{tab:PredictionVariousModels}
\end{table}
